A reliable order-statistics-based approximate nearest neighbor search algorithm

We propose a new algorithm for fast approximate nearest neighbor search based on the properties of ordered vectors. Data vectors are classified based on the index and sign of their largest components, thereby partitioning the space in a number of cones centered in the origin. The query is itself classified, and the search starts from the selected cone and proceeds to neighboring ones. Overall, the proposed algorithm corresponds to locality sensitive hashing in the space of directions, with hashing based on the order of components. Thanks to the statistical features emerging through ordering, it deals very well with the challenging case of unstructured data, and is a valuable building block for more complex techniques dealing with structured data. Experiments on both simulated and real-world data prove the proposed algorithm to provide a state-of-the-art performance.

==> Biographies.tex <==

{Luisa Verdoliva}
is Assistant Professor of Telecommunications
with the Department of Electrical Engineering and Information Technology of the University University of Naples Federico II, Naples, Italy.
Her research is on image processing, in particular compression and restoration of remote-sensing images, both optical and SAR, and digital forensics.
Dr. Verdoliva has been elected member of the IEEE Information Forensics and Security Technical Committee for the 2016-2018 period.

{Davide Cozzolino}
received the Laurea degree in computer engineering and the Ph.D. degree in information engineering 
from the University Federico II of Naples, Italy, in December 2011 and April 2015, respectively.
He is currently a Post Doc at the same University.
His study and research interests include image processing, particularly forgery detection and localization.

{Giovanni Poggi}
is Full Professor of Telecommunications and vice Director of the
Department of Electrical Engineering and Information Technology of the University University of Naples Federico II, Naples, Italy.
His research interests are in statistical image processing, including compression, restoration, segmentation, and classification,
with application to remote-sensing, both optical and SAR, digital forensics, and biometry.
Prof. Poggi has been an Associate Editor for the IEEE Transactions on Image Processing and Elsevier Signal Processing


\end{document}


==> Contact_Info.tex <==

Luisa Verdoliva
DIETI
University Federico II of Naples, Naples, ITALY
+39 081 7683929
verdoliv@unina.it

Davide Cozzolino
DIETI
University Federico II of Naples, Naples, ITALY
+39 081 7683839
davide.cozzolino@unina.it

Giovanni Poggi
DIETI
University Federico II of Naples, Naples, ITALY
+39 081 7683151
poggi@unina.it


